Generative Unlearning for Any Identity

Recent advances in generative models trained on large-scale datasets have made it possible to synthesize high-quality samples across various domains. Moreover, the emergence of strong inversion networks enables not only a reconstruction of real-world images but also the modification of attributes through various editing methods. However, in certain domains related to privacy issues, e.g., human faces, advanced generative models along with strong inversion methods can lead to potential misuses. In this paper, we propose an essential yet under-explored task called generative identity unlearning, which steers the model not to generate an image of a specific identity. In the generative identity unlearning, we target the following objectives: (i) preventing the generation of images with a certain identity, and (ii) preserving the overall quality of the generative model. To satisfy these goals, we propose a novel framework, Generative Unlearning for Any Identity (GUIDE), which prevents the reconstruction of a specific identity by unlearning the generator with only a single image. GUIDE consists of two parts: (i) finding a target point for optimization that un-identifies the source latent code and (ii) novel loss functions that facilitate the unlearning procedure while less affecting the learned distribution. Our extensive experiments demonstrate that our proposed method achieves state-of-the-art performance in the generative machine unlearning task. The code is available at https://github.com/KHU-AGI/GUIDE.

==> sec/0_abstract_feedback.tex <==
\begin{abstract}
How can we make the generative models forget to generate us?
Recent advances in generative models based on large-scale datasets have made it possible to synthesize high-quality samples in \sj{various} domains.
\sj{Moreover, the emergence of strong inversion networks enables not only a reconstruction of real-world images but also a modification of} attributes through various editing methods.
\sj{However, in certain domains related to privacy issues, \eg, human faces, this can lead to potential misuse.}
In this paper, we propose \sj{an essential yet under-explored} task called generative machine unlearning, \sj{which steers the model not to generate a specific identity.}
In the generative machine unlearning, \sj{we target the followings;}
(\lowercase{\romannumeral1}) \sj{To prevent the generation of images with a certain identity}, and (\lowercase{\romannumeral2}) to preserve the overall generation quality.
To satisfy these concerns, we propose a novel framework, MUG, \sj{which prevents the reconstruction of a specific identity by unlearning the generator with a single image of the given identity}.
We construct MUG in two parts:
% We shift the latent code corresponding to the identity we want to unlearn to another latent code in the model.
\sj{(\lowercase{\romannumeral1}) latent shifting module that} shifts the latent code corresponding to the identity and \sj{(\lowercase{\romannumeral2}) generator preservation module that helps to maintain the performance of} the existing generator.
\sj{We} demonstrated that \sj{our proposed method} achieves state-of-the-art performance in the proposed generative machine unlearning task via extensive experiments.
% It indicates that the proposed MUG can remove a certain identity successfully, while not intervening the overall generation performance.
The code will be released after the review.
\end{abstract}

==> sec/0_abstract_old.tex <==
\begin{abstract}
How can we make the generative models forget to generate us?
Recent advances in generative models based on large-scale datasets have made it possible to synthesize high-quality samples in \sj{various} domains.
However, in certain domains, especially human faces, this achievement leads to potential misuse. 
Anyone can easily represent a specific identity in a model through the inversion networks, and then easily modify attributes through the editing methods.
To prevent the creation of a specific identity in a generative model, in this paper, we propose a challenging task called generative machine unlearning.
In generative machine unlearning task, there are two things to consider.
The first is to remove certain identities from the generative model, and the second is to preserve the overall generation quality.
To satisfy these concerns, we propose a novel framework, MUG.
We construct MUG from two parts.
We shift the latent code corresponding to the identity we want to unlearn to another latent code in the model.
At the same time, we preserve the existing generation of uninteresting latent codes.
Extensive experiments demonstrate that the proposed MUG achieve state-of-the-art performance in the proposed generative machine unlearning task.
It indicates that the proposed MUG can remove a certain identity successfully, while not intervening the overall generation performance.
The code will be released after the review.
\end{abstract}

==> sec/1_intro_feedback.tex <==
\section{Introduction}
\sj{Recent models with large-scale pre-training, \eg, CLIP \cite{radford2021learning}, \textbf{write more examples}, have been remarkably changed the landscape of deep learning.}
\sj{In specific, deep generative models,} \eg, generative adversarial networks (GANs) \cite{goodfellow2014generative, Karrs2018progressive,karras2019style} and Diffusion models \cite{ho2020denoising,song2019generative}, are \sj{notably affected by abundant usage of data, and show outstanding performance in a wide range of applications with generating high-fidelity realistic images.}
However, this progress has raised concerns regarding the potential misuse of models, \sj{which is mainly related to user privacy by reversely tracking the dataset used for training}, \eg, membership inference attack \cite{shokri2017membership}, or model inversion attack \cite{fredrikson2015model}.
With increasing awareness of user privacy, various privacy regulations have been implemented, providing individuals with control over their personal data.
For instance, the European Union has established the General Data Protection Regulation (GDPR) \cite{voigt2017eu}, which emphasizes "\textit{the right to be forgotten}".
\sj{These regulations are closely related to \textit{Machine Unlearning} \cite{xu2023machine}, which} involves the removal of specific knowledge or the erasure of the influence of certain, \eg, harmful, private, or biased, data from the training dataset of pre-trained models. 
Achieving this often requires extensive retraining, presenting challenges in terms of time and computational resources.
Thus, innovative and efficient techniques are introduced to selectively forget information for machine unlearning \cite{golatkar2020eternal,golatkar2020forgetting,mehta2022deep, peste2021ssse}.

Nevertheless, \sj{still the majority of existing machine unlearning methods have been primarily focused on supervised tasks.}
% indicating a need for broader exploration and application of this concept across various domains of machine learning.
% In the generative tasks, on the other hand, machine unlearning is more necessary.
\sj{However, with the emergence of robust inversion models \cite{richardson2021encoding, tov2021designing, roich2022pivotal, moon2022interestyle, yuan2023make, wang2022high} combined with powerful pre-trained generators \cite{karras2019style, karras2020analyzing, chan2022efficient}, one can easily reconstruct the image with a specific identity via deep learning models.}
Furthermore, the reconstructed image can be manipulated or edited easily \sj{via robust image editing methods \cite{shen2020interpreting, patashnik2021styleclip, shen2020interfacegan}, which can generate malicious fake information.}
This can lead to many exploits such as deepfake and other illegal content.

% However, many approaches merely focus on detecting whether the given images or videos are deepfake or not \cite{xu2023tall, yan2023ucf}.
% No approaches have been explored to prevent the generative models themselves from generating someone.

% Machine unlearning in GM & Our task
There have been several attempts to adapt machine unlearning in the field of generative models \cite{gandikota2023erasing,kumari2023ablating,moon2023feature,tiwary2023adapt} to prevent abuse of explicit contents or change facial features.
However, most of these efforts have focused only on unlearning high-level concepts, \sj{instead of privacy protection}, containing facial features, explicit content such as "Nudity" or the style of renowned artists like "Van Gogh".
\sj{Consequently, the pre-mentioned unlearning methods are not adequate to refrain from the malicious usage of generative models via inversion and editing.}
% Unlearning features or styles do not directly address privacy concerns related to the misuse of individual identity such as deep fake or face manipulation.
\sj{Instead, the unlearning method should enable the complete unlearning of the identity of a specific person from the model rather than partial features.}
 
In this paper, we tackle the novel problem of unlearning identity from pre-trained GANs.
We assume the real-world situation \sj{which targets unlearning the whole specific identity from the generator, only utilizing the single image of the given identity.}
\sj{We note that this is a more challenging task than typical unlearning scenarios, \textbf{please write down details of typical unlearning scenarios.}
}
The contributions of our paper are:
\begin{itemize}
    \item First, we tackle machine unlearning in generative models \sj{in the aspect of privacy protection}.
    In our task, we aim to prevent the pre-trained generative models from synthesizing someone's identity.
    \sj{To the best of our knowledge, our method is the first to tackle the privacy issue of the unconditional generative models.}
    \item Contribution 2
    \item \sj{We demonstrated that our proposed framework can remove the specific identity successfully in the generative model while minimizing} the effect on other identities. Moreover, we showed that our framework achieves state-of-the-art performance both qualitatively and quantitatively, \sj{through extensive experiments.}
\end{itemize}

==> sec/1_intro_old.tex <==
\section{Introduction}
% Recent trend and Privacy concern
The landscape of deep learning has been significantly transformed by the advent of large-scale pre-trained generative models \cite{ramesh2022hierarchical}.
Consequently, recent advancements in deep generative models, including generative adversarial networks (GANs) \cite{goodfellow2014generative,Karrs2018progressive,karras2019style} and Diffusion models \cite{ho2020denoising,song2019generative}, have been demonstrated to show outstanding performance in a wide range of applications, notably in generating high-fidelity realistic images.
However, this progress has raised concerns regarding the potential misuse of models such as membership inference attack \cite{shokri2017membership} or model inversion attack \cite{fredrikson2015model}.
With increasing awareness of user privacy, various privacy regulations have been implemented, providing individuals with control over their personal data.
For instance, the European Union has established the General Data Protection Regulation (GDPR) \cite{voigt2017eu}, which emphasizes "\textit{the right to be forgotten}".
% In some cases, generated images might include violent or explicit content and unintentionally reveal private information used in training the model.

% Machine unlearning definition and applications
Due to above-mentioned concerns, Machine Unlearning \cite{xu2023machine} has emerged as a crucial area of focus.
Machine unlearning involves the removal of specific knowledge or the erasure of the influence of certain data from the training dataset of pre-trained models, particularly data that is harmful, private, or biased. 
Achieving this often requires extensive retraining, presenting challenges in terms of time and computational resources.
Thus, innovative and efficient techniques are introduced to selectively forget information for machine unlearning \cite{golatkar2020eternal,golatkar2020forgetting,mehta2022deep, peste2021ssse}.
Nevertheless, it is important to note that the majority of existing machine unlearning methods have been primarily focused on supervised tasks, indicating a need for broader exploration and application of this concept across various domains of machine learning.

% Necessity of machine unlearning in GM
In the generative tasks, on the other hand, machine unlearning is more necessary.
For example, based on the powerful generation ability of the pre-trained generative models \cite{karras2019style, karras2020analyzing, chan2022efficient}, one can easily represent someone in the generative models \cite{richardson2021encoding, tov2021designing, roich2022pivotal, moon2022interestyle, yuan2023make}.
Moreover, the represented identities can be further manipulated or edited easily \cite{shen2020interpreting, patashnik2021styleclip}.
This can lead to many exploits such as deepfake and other illegal contents.

% However, many approaches merely focus on detecting whether the given images or videos are deepfake or not \cite{xu2023tall, yan2023ucf}.
% No approaches have been explored to prevent the generative models themselves from generating someone.

% Machine unlearning in GM & Our task
There have been several attempts to adapt machine unlearning in the field of generative models \cite{gandikota2023erasing,kumari2023ablating,moon2023feature,tiwary2023adapt} to prevent abuse of explicit contents or change facial features.
However, most of these efforts have focused only on unlearning high-level concepts containing facial features, explicit contents such as "Nudity" or style of renowned artists like "Van Gogh".
Unlearning features or styles does not directly address privacy concerns related to the misuse of individual identity such as deep fake or face manipulation.
To directly address privacy issues, it becomes crucial to completely unlearn the identity of a specific person from the model rather than partial features.
 
In this paper, we tackle the novel problem of unlearning identity from pre-trained GANs.
We assume the real-world situation where only one image of the user is given, making it a more challenging task than typical unlearning scenarios, as training data for unlearning the user's facial information is not available.

The contributions of our paper are:
\begin{itemize}
    \item To the best of our knowledge, we tackle machine unlearning in generative models. In our task, we aim to prevent the pre-trained generative models from synthesizing someone's identity.
    \item Contribution 2
    \item Extensive experiments demonstrate that our proposed framework can remove someone's identity successfully in the generative model while having less effect on the other identities. Moreover, our framework achieves state-of-the-art performance both qualitatively and quantitatively.
\end{itemize}

==> sec/3_method_feedback.tex <==
\input{fig/fig_structure}
\section{Method}
\subsection{Problem Formulation}
\label{sec:problem_formulation}
% Given a set of images $\mathbf{x}$ depicting a specific identity, we designate an image $x_u$ as an exemplar of that identity and refer to it as a source image.
Given a set of images $\mathbf{x}$ depicting a specific identity, \sj{we randomly select a single source image $x_u\in\mathbf{x}$ as an exemplar of the identity.}
% Initially, we embed $x_u$ to derive $w_u$ in the latent space of the 3D GAN generator, specifically EG3D, utilizing an off-the-shelf GAN inversion network $E$ \cite{yuan2023make}:
\sj{Initially, using off-the-shelf inversion network \cite{yuan2023make} $E$ corresponding to the unconditional generator, \ie, EG3D \cite{chan2022efficient}, we embed $x_u$ to the source latent code $w_u$ in the latent space of EG3D:}
\begin{align}\label{eqn:inversion}
w_u = E(x_u)
\end{align}

\sj{Since EG3D \cite{chan2022efficient} consists of the mapping network $\mathrm{MLP}(\cdot)$, StyleGAN2 \cite{karras2019style} backbone $G(\cdot)$ and the neural renderer with a super-resolution module $R(\cdot)$, we can denote the reconstructed image $\hat{x}$ from $w_u$ as following:}

\begin{align}
\hat{x} = R(G(w_u); c),
\end{align}
where $c$ denotes camera poses.
For convenience, we omit the explicit notation of camera poses in this paper, \sj{\ie, $\hat{x} = (R \circ G)(w_u)$.}
\sj{We target to} derive an unlearned \sj{$G$}, \ie, $G_u$, from the pre-trained EG3D generator $G$, \ie, $G_s$, \sj{while fixing $\mathrm{MLP}$ and $R$.
With proper unlearning, an image generated by unlearned EG3D using $w_u$, \ie, $\hat{x}_u = (R \circ G_u)(w_u)$ should have a distinct identity from the image generated by original EG3D using $w_u$, \ie, $(R \circ G_s)(w_u)$.}

In our task formulation, two considerations are paramount;
Firstly, we aim to eliminate the entire identity from the generator \sj{only utilizing a single image}.
To validate this, we incorporate a test image $x_{test}\in\mathbf{x}$ and its corresponding latent code \sj{$w_{test}$, \ie, $w_{test} = E(x_{test})$.}
\sj{By utilizing $x_{test}$, we can verify whether the generator successfully unlearns the identity rather than unlearn only $x_{u}$.}
Secondly, we strive to maintain the generation performance of the pre-trained model.
To assess this, we sample multiple images from fixed latent codes using both the unlearned and pre-trained generators.
Subsequently, we estimate the distribution shift between the images before and after the unlearning process.


\subsection{\sj{Un-identifying Face On Latent Space}}
\label{method:ufo}

\sj{The successfully unlearned model should not generate the image with the identity of $\mathbf{x}$, even when $w_u$ is used as a latent.
Consequently, we initiate our approach to manipulate $\hat{x}_u$ to be another image rather than the image with identity in $\mathbf{x}$ by unlearning $G$.
To design the objective function for unlearning, firstly we need to set the goal unlearned image $\hat{x}_t$ that $\hat{x}_u$ should mimic after unlearning.
While there exist various options for setting $\hat{x}_t$, \eg, a random face or even a non-human image, we choose the mean face generated by the mean latent $\Bar{w}$ of $\mathrm{MLP}$, \ie, $(R \circ G_s)(\Bar{w})$, as $\hat{x}_t$.
This setting is inspired by inversion methods \cite{alaluf2021restyle, moon2022interestyle} which apply the identity to the mean face through inversion stages.
Since our goal is to un-identify the image, we argue that it is intuitive and reasonable to send the image back to the mean face, which is opposite to the inversion.
}

However, \sj{this simple approach might be problematic} when $w_u$ is close to $\Bar{w}$, where the unlearned image might still resemble the original identity.
\sj{To this end, we propose a novel method named Un-identifying Face On latent space (UFO), which can set $\hat{x}_t$ robustly regardless of the distance between $w_{u}$ and $\Bar{w}$.
The following are the processes of UFO:
First, by subtracting $\Bar{w}$ from $w_{u}$, we extract the identity latent $w_{id} = w_{u}-\Bar{w}$.
}
Then we propose a process of \textit{en}-identification, setting the target in the opposite direction of the existing $w_{id}$ to foster a more pronounced change in identity, creating an entirely new identity.
\sj{In other words,} we chose $\Bar{w}$ as the stopover point and established the final target point at the extrapolation of $w_u$ and $\Bar{w}$.
The finalized target point can be expressed as
\begin{align}
w_t = \Bar{w} -  d \cdot \frac{w_{i d}}{\left\|w_{i d}\right\|_2},
\end{align}
where $d$ is defined as the distance that balances identity and FID, as determined by our empirical results.
\sj{Finally, we can set $\hat{x}_t=(R \circ G_s)(w_t)$}.

\subsection{Latent Space Distortion}
\label{method:lsd}
\sj{
After setting $\hat{x}_t$, we need to robustly design the unlearning process that can effectively make $\hat{x}_u$ to be similar to $\hat{x}_t$, while maintaining the generation performance of $G_u$.
We coin this process as Latent Space Distortion (LSD), which targets to unlearn images from the specific latent while keeping generation results from other latents.
LSD utilizes the following three losses to achieve this goal:
}

\paragraph{Local Unlearning Loss.}
\sj{To force $\hat{x}_u$ to be $\hat{x}_t$, we use the widely-used reconstruction losses, \ie, Euclidean loss $\mathcal{L}_{2}$, perceptual loss \cite{zhang2018unreasonable} $\mathcal{L}_{per}$, and identity loss \cite{deng2019arcface} $\mathcal{L}_{id}$.
Using $\mathcal{L}_{recon}$}, we compare the tri-plane features $F_u = G_u(w_u)$ and $F_t = G_s(w_t)$, originating from the source and target latent codes, respectively.
The local unlearning loss function is defined as;
\begin{align}
\label{eq:local}
        &\mathcal{L}_{local}(\hat{x}_u, \hat{x}_t) = \\
        &\lambda_{L2}\mathcal{L}_{L2}(F_u, F_t) + \lambda_{per}\mathcal{L}_{per}(\hat{x}_u, \hat{x}_t)
        + \lambda_{id}\mathcal{L}_{id}(\hat{x}_u, \hat{x}_t).
\end{align}

\paragraph{Adjacency-Aware Unlearning Loss.}
The above equation considers only one pair of source and target latent codes.
However, images \sj{of similar identity with} the source identity can be obtained by introducing \sj{marginal} perturbations to the latent code.
For the successful unlearning of the given identity, we need to consider the neighborhood of both the source and the target latent codes.
Consequently, we sample $N_a$ latent codes \sj{in the vicinity of} the $w_u$.
Specifically, with the hyperparameter $\alpha$, \sj{we define} the distances $\Delta$ to compute the adjacent latent codes as:

\begin{align}
    \Delta = \{\alpha \cdot \frac{w^i_{r,a} - w_u}{\Vert w^i_{r,a} - w_u \Vert_2}\}^{N_a}_{i=1},
\end{align}

where $w^i_{r,a}$ is a latent code sampled from the random noise vector $z^i_{r,a}$.
Using these distances $\Delta$, we can compute $N_a$ latent codes for both the source and the target latent codes.
Similar to the local unlearning loss, we optimize the \sj{generated triplane features and images from} $w^i_{u,a} = w_u + \Delta^i$ and $w^i_{t,a} = w_t + \Delta^i$ to be similar:

\begin{align}
    &\hat{x}^i_{u,a} = R(F^i_{u,a}), \hat{x}^i_{t,a} = R(F^i_{u,a}),\\
    &
        \mathcal{L}_{adj}(w_u, w_t) = \cfrac{1}{N_a}\sum\limits^{N_a}_{i=1}\mathcal{L}_{local,a}(\hat{x}^i_{u,a}, \hat{x}^i_{t,a}),
\end{align}
\sj{where $F^i_{u,a} = G_u(w^i_{u,a}), F^i_{t,a} = G_s(w^i_{t,a})$ denotes for triplane features, and $\mathcal{L}_{local,a}$ for the same loss in equation \ref{eq:local}, but only with different $\lambda_{L2}$, and $\lambda_{per}$, and $\lambda_{id}$.
}

\paragraph{Global Preservation Loss.}
While the local unlearning loss and adjacency-aware unlearning loss mentioned above facilitate the removal of the source identity, we propose a global preservation loss to mitigate side effects arising from these unlearning loss functions.
In the global preservation loss, we constrain the generator to maintain generation performance for latent codes that are relatively distant from both the source and target latent codes.

To be precise, we sample $N_g$ latent codes $\{w^i_{r,g}\}^{N_g}_{i=1}$ from random noise vectors $\{z^i_{r,g}\}^{N_g}_{i=1}$.
We ensure that these latent codes do not overlap with the adjacent latent codes used in the adjacency-aware unlearning loss.
Unlike the unlearning loss functions, we find that adopting only perceptual loss achieves a balanced performance between identity shift and model preservation.
The global preservation is computed as:

\begin{align}
&\begin{array}{cc}
\hat{x}^i_{u,g} = (R \circ G_u)(w^i_{r,g}), \\
\hat{x}^i_{s,g} = (R \circ G_s)(w^i_{r,g}), \\
\end{array} \\
&\mathcal{L}_{global}(G_u, G_s) = \cfrac{1}{N_g}\sum\limits^{N_g}_{i=1}\mathcal{L}_{per}(\hat{x}^i_{u,g}, \hat{x}^i_{s,g}).
\end{align}

In summary, our final objective is:
\sj{
\begin{align}
&\mathcal{L}(\hat{x}_u, \hat{x}_t, w_u, w_t, G_u, G_s) = \\
&\mathcal{L}_{local}(\hat{x}_u, \hat{x}_t) + \lambda_{adj}\mathcal{L}_{adj}(w_u, w_t) + \lambda_{global}\mathcal{L}_{global}(G_u, G_s).
\end{align}
}

==> sec/3_method_old.tex <==
\section{Method}
\subsection{Problem Formulation}
\label{sec:problem_formulation}
% Given a set of images $\mathbf{x}$ depicting a specific identity, we designate an image $x_u$ as an exemplar of that identity and refer to it as a source image.
Given a set of images $\mathbf{x}$ depicting a specific identity, \sj{we randomly select a single source image $x_u\in\mathbf{x}$ as an exemplar of the identity.}
% Initially, we embed $x_u$ to derive $w_u$ in the latent space of the 3D GAN generator, specifically EG3D, utilizing an off-the-shelf GAN inversion network $E$ \cite{yuan2023make}:
\sj{Initially, using off-the-shelf inversion network \cite{yuan2023make} $E$ corresponding to the unconditional generator, \ie, EG3D \cite{chan2022efficient}, we embed $x_u$ to the source latent code $w_u$ in the latent space of EG3D:}
\begin{align}\label{eqn:inversion}
w_u = E(x_u) % need to modification + \Bar{w}.
\end{align}

% We term $w_u$ as the source latent code.
% In the EG3D architecture, the generator comprises three components: the mapping network $\mathrm{MLP}(\cdot)$, the StyleGAN2 generator $G(\cdot)$, and the neural render with a super-resolution module $R(\cdot)$. Consequently, we can reconstruct an image from the source latent code $w_u$ as follows:
\sj{Since EG3D \cite{chan2022efficient} consists of the mapping network $\mathrm{MLP}(\cdot)$, StyleGAN2 \cite{karras2019style} backbone $G(\cdot)$ and the neural renderer with a super-resolution module $R(\cdot)$, we can denote the reconstructed image $\hat{x}_u$ from $w_u$ as following:}

\begin{align}
\hat{x}_u = R(G(w_u); c),
\end{align}
where $c$ denotes camera poses.
For convenience, we omit the explicit notation of camera poses in this paper, \sj{\ie, $\hat{x}_u = (R \circ G)(w_u)$.}
% We fix the mapping network and the neural render with the super-resolution module from the pre-trained source EG3D generator.
% $G_u$ should produce an image from the source latent code, denoted as $(R \circ G_u)(w_u)$, representing a distinct identity from $(R \circ G_s)(w_u)$.
\sj{We target to} derive an unlearned \sj{$G$}, \ie, $G_u$, from the pre-trained EG3D generator $G$, \ie, $G_s$, \sj{while fixing $\mathrm{MLP}$ and $R$.
With proper unlearning, an image generated by unlearned EG3D using $w_u$, \ie, $(R \circ G_u)(w_u)$ should have a distinct identity from the image generated by original EG3D using $w_u$, \ie, $(R \circ G_s)(w_u)$.}

In our task formulation, two considerations are paramount;
Firstly, we aim to eliminate the entire identity from the generator \sj{only utilizing a single image}.
To validate this, we incorporate a test image $x_{test}\in\mathbf{x}$ and its corresponding latent code \sj{$w_{test}$, \ie, $w_{test} = E(x_{test})$.}
% This allows us to verify if the generator successfully discards the provided identity, accounting for variations in background, poses, or styles.
\sj{By utilizing $x_{test}$, we can verify whether the generator successfully unlearns the identity rather than unlearn only $x_{u}$.}
Secondly, we strive to maintain the generation performance of the pre-trained model.
To assess this, we sample multiple images from fixed latent codes using both the unlearned and pre-trained generators.
Subsequently, we estimate the distribution shift between the images before and after the unlearning process.
% In this section, we first formulate the generative unlearning task that we are proposing to tackle.
% There is a set of images $\mathbf{x}$, which contains images of an identity of someone.
% We split this set into an source image $x_u$ which is used for unlearning and the test set $\mathbf{x}_{test}$ of the size $N_{test}$, where $x_u \notin \mathbf{x}_{test}$.
% We use the unlearning image to eliminate the generator's ability to generate the identity of $\mathbf{x}$.
% And we evaluate whether the unlearning process is successful by using the test set $\mathbf{x}_{test}$.

% In the unlearning process, we embed a image in $x_u$ into the pre-trained source generator network $G_s$ by using GAN inversion methods $G^{-1}$ to obtain the corresponding latent codes $w_u$: 
% \begin{align}
%     w_u = G^{-1}(x_u),
% \end{align}
% where $w_u \in \mathcal{W}^{+}$.
% The goal in this unlearning process is to obtain the unlearned generator $G_u$ which can not generate the images of the identities that are similar to $\mathbf{x}_u$.

% In the test process, our main concerns are twofold.
% The first is to verify that the unlearning process successfully de-identified the unseen images.
% To verify this, we leverage the test set $\mathbf{x}_{test}$ and we embed the images in $\mathbf{x}_{test}$ into $\mathbf{w}_{test} =\{w^{i}_t\}^{N_{test}}_{i=1}$:
% \begin{align}
%     \mathbf{w}_{test} = G^{-1}(\mathbf{x}_{test}),
% \end{align}
% where $\mathbf{w}_{test} \in \mathcal{W}^{+}$.
% We evaluate whether the images from the unlearned generator with the camera poses $\mathbf{c}$ - $G_u(\mathbf{w}_{test},\mathbf{c})$ are retaining the identity of $\mathbf{x}_{test}$.

% Second, we want to make sure that the unlearning process doesn't harm the overall performance of the model.
% To check this, we sample $N_p$ latent codes $ \mathbf{w}_p=\{{w^i_p} \}^{N_p}_{i=1}$.
% They are the outputs of the mapping network \cite{chan2022efficient} from random noise vectors $\mathbf{z}_p=\{z^i_p\}^{N_p}_{i=1}$ conditioned on the camera poses $\mathbf{c}$:
% \begin{align}
%     \mathbf{w}_p = \mathrm{MLP}(\mathbf{z}_p;\mathbf{c}),
% \end{align}
% where $\mathrm{MLP}$ denotes mapping network, $\mathbf{z}_p \in \mathcal{Z}$ and $\mathbf{w}_p \in \mathcal{W}^+$.
% To embed an image into our generator network, we invert the image into an latent code $w_{u,i} \in \mathcal{W}^{+}$ using GAN inversion methods:
% \begin{align}
%     w_{u,i} = G^{-1}(x_{u,i}).
% \end{align}
% On the other hand, there are $N_p$ latent codes $ \mathbf{w}_p=\{{w^i_p} \}^{N_p}_{i=1}\in\mathcal{W}^{+}$.
% They are the outputs of the mapping network \cite{chan2022efficient} from random noise vectors $\mathbf{z}_p=\{z^i_p\}^{N}_{i=1} \in \mathcal{Z}$ conditioned on the camera poses $\mathbf{c}=\{c^i\}^N_{i=1}$:
% \begin{align}
%     \mathbf{w}_p = \mathrm{Mapping}(\mathbf{z}_p;\mathbf{c}).
% \end{align}
% One can synthesize images $\hat{x}_u$ and $\hat{\mathbf{x}}_p$ corresponding to $w_u$ and $\mathbf{w}_p$ by using generator $G$ and the camera poses $c'$ and $\mathbf{c}$, respectively:
% \begin{align}
%     \hat{x}_u = G(w_u, c'), \hat{\mathbf{x}}_p = G(\mathbf{w}_p, \mathbf{c})
% \end{align}
% For the image of a certain identity (with a subscript of $u$), we call this an unlearning target.
% Our goal is to make the generator $G$ not synthesize images similar to the original unlearning target image $x_u$ while retaining the generation abilities for the others (with a subscript of $p$).
% We check if the images from the pre-trained source generator $G_s(\mathbf{w}_p, \mathbf{c})$ and the unlearned generator $G_u(\mathbf{w}_p, \mathbf{c})$ are visually same.
% For detailed evaluation protocols, please refer Section \ref{sec:experimental_setup}.

\begin{figure*}
    \includegraphics[width=\textwidth]{figures/main_figure.pdf}
    \vspace{-0.7cm}
    \caption{In the context of identity unlearning, the foremost priority is to find an adequate target point. We initiate our approach by analyzing the source latent codes derived through GAN inversion.In the context of identity unlearning, the foremost priority is to find an adequate target point. We initiate our approach by analyzing the source latent codes derived through GAN inversion.}
\end{figure*}

\subsection{\sj{Unidentifying Face On Latent Space}}
In the context of identity unlearning, the foremost priority is to find an adequate target \sj{latent}.
We initiate our approach by analyzing \sj{$w_u$} derived through GAN inversion.
\sj{With utilizing the mean latent }$\Bar{w}$, \ie, the average latent code of $\mathrm{MLP}(z)$ from random noise vector $z$, $w_u$ \sj{can be represented as a combination of $\Bar{w}$ and identity latent, $w_{id}$}:
\begin{align}
w_u = \Bar{w} + w_{id},
\end{align}
% where $\Bar{w}$ indicates the average latent code of $\mathrm{MLP}(z)$ from random noise vector $z$ and $w_{id}$ implies the latent code extracted from the source image $x_u$ during the inversion process.
Since $\Bar{w}$ plays a role representing the face with base identity, we can assume that $w_{id}$ possesses the identity information of $x_u$.

Based on the analysis of $w_u$, we determined that diminishing the influence of identity information of $x_u$ is directly essential for the success of identity unlearning.
Thus, we considered $\Bar{w}$ as our target point for the \textit{de}-identification process in the generator.
However, a challenge emerges when $w_u$ is close to $\Bar{w}$, which can hinder the unlearning of the source identity.
Therefore, we propose a process of \textit{en}-identification, setting the target in the opposite direction of the existing $w_{id}$ to foster a more pronounced change in identity, creating an entirely new identity.
Consequently, we chose $\Bar{w}$ as the stopover point and established the final target point at the extrapolation of $w_u$ and $\Bar{w}$.
The finalized target point can be expressed as
\begin{align}
w_t = \Bar{w} -  d \cdot \frac{w_{i d}}{\left\|w_{i d}\right\|_2},
\end{align}
where $d$ is defined as the distance that balances identity and FID, as determined by our empirical results.

% Based on the analysis of source latent codes, we determine the stopover point as $\Bar{w}$ for the de-identification process of $G_s$.
% A problem arises when $w_u$ is close to $\Bar{w}$, impeding the unlearning of the source identity.
% Consequently, we establish the final target point at the extrapolation of $w_u$ and $\Bar{w}$.
% The en-identification process involves optimizing towards this target point, which is in the opposite direction of $w_{id}$, expressed as
% \begin{align}
% w_t = \Bar{w} -  d \cdot \frac{w_{i d}}{\left\|w_{i d}\right\|_2},
% \end{align}
% where $d$ is defined as the optimal distance that balances identity and FID, as determined by our experiments.

% From this, we can easily infer that $E(x_u)$ represents the identity of input image $x_u$.
% To achieve our unlearning goal, we need to do de-identification process for removing specific identity and, based on above insight, we remove specific identity like:
% \begin{align}
% \Bar{w} + w_d \to \Bar{w}
% \end{align}
% However, in harsh case, we imagine that if input image is similar with $\Bar{w}$ then above method cannot well unlearn target image from pre-trained model.
% To solve this problem, we propose extrapolation target.

\subsection{Loss Functions}
Building upon the target latent code $w_t$ discussed in the previous section, we now elaborate on the loss functions employed in our unlearning process.
To achieve this, we employ the pre-trained and fixed source generator $G_s$ to sample either a tri-plane feature map $F_t$ or an image $\hat{x}_t$ from the target latent code.
\paragraph{Local Unlearning Loss.}
To replace the source identity with the target identity, we employ fundamental and widely-used loss functions, namely reconstruction loss, perceptual loss, and identity loss.
In the case of the reconstruction loss, we compare the tri-plane features $G_u(w_u)$ and $G_s(w_t)$, originating from the source and target latent codes, respectively.
The local unlearning loss function is given by:
\begin{align}
    &\begin{array}{cc}
        F_u = G_u(w_u), F_t = G_s(w_t),
    \end{array} \\
    &\begin{array}{cc}
        \hat{x}_u = R(F_u), \hat{x}_t = R(F_t), 
    \end{array} \\
    &\begin{array}{cc}
        \mathcal{L}_{local} = \lambda_{L2}\mathcal{L}_{L2}(F_u, F_t) + \lambda_{per}\mathcal{L}_{per}(\hat{x}_u, \hat{x}_t)\\
        + \lambda_{id}\mathcal{L}_{id}(\hat{x}_u, \hat{x}_t),
    \end{array}
\end{align}
where $\mathcal{L}_{per}$ refers to perceptual loss \cite{zhang2018unreasonable}, and $\mathcal{L}_{id}$ denotes identity loss \cite{deng2019arcface}.
\paragraph{Adjacency-Aware Unlearning Loss.}
The above equation considers only one pair of source and target latent codes. 
However, similar images of the source identity can be obtained by introducing perturbations to the latent code.
For the successful unlearning of the given identity, we need to consider the neighborhood of both the source and the target latent codes. 
Consequently, we sample $N_a$ latent codes near the source latent code.
Specifically, with the hyperparameter $\alpha$, the distances $\Delta$ to compute the adjacent latent codes are defined as:

\begin{align}
    \Delta = \{\alpha \cdot \frac{w^i_{r,a} - w_u}{\Vert w^i_{r,a} - w_u \Vert_2}\}^{N_a}_{i=1},
\end{align}

where $w^i_{r,a}$ is a latent code sampled from the random noise vector $z^i_{r,a}$.
Using these distances $\Delta$, we can compute $N_a$ latent codes for both the source and the target latent codes.
Similar to the local unlearning loss, we optimize the generator to behave as $w_u + \Delta^i$ for $w_t + \Delta^i$:

\begin{align}
    &w^i_{u,a} = w_u + \Delta^i,  w^i_{t,a} = w_t + \Delta^i,\\
    &F^i_{u,a} = G_u(w^i_{u,a}), F^i_{t,a} = G_s(w^i_{u,a}),\\
    &\hat{x}^i_{u,a} = R(F^i_{u,a}), \hat{x}^i_{t,a} = R(F^i_{u,a}),\\
    &\begin{array}{cc}
        \mathcal{L}_{adj} = \cfrac{1}{N_a}\sum\limits^{N_a}_{i=1}\{\lambda^a_{L2}\mathcal{L}_{L2}(F^i_{u,a}, F^i_{t,a}) \\
        + \lambda^a_{per}\mathcal{L}_{per}(\hat{x}^i_{u,a}, \hat{x}^i_{t,a}) + \lambda^a_{id}\mathcal{L}_{id}(\hat{x}^i_{u,a}, \hat{x}^i_{t,a})\}.
    \end{array}
\end{align}
\paragraph{Global Preservation Loss.}
While the local unlearning loss and adjacency-aware unlearning loss mentioned above facilitate the removal of the source identity, we propose a global preservation loss to mitigate side effects arising from these unlearning loss functions.
In the global preservation loss, we constrain the generator to maintain generation performance for latent codes that are relatively distant from both the source and target latent codes.

To be precise, we sample $N_g$ latent codes $\{w^i_{r,g}\}^{N_g}_{i=1}$ from random noise vectors $\{z^i_{r,g}\}^{N_g}_{i=1}$.
We ensure that these latent codes do not overlap with the adjacent latent codes used in the adjacency-aware unlearning loss.
Unlike the unlearning loss functions, we find that adopting only perceptual loss achieves a balanced performance between identity shift and model preservation.
The global preservation is computed as:

\begin{align}
&\begin{array}{cc}
\hat{x}^i_{u,g} = (R \circ G_u)(w^i_{r,g}), \\
\hat{x}^i_{s,g} = (R \circ G_s)(w^i_{r,g}), \\
\end{array} \\
&\mathcal{L}_{global} = \cfrac{1}{N_g}\sum\limits^{N_g}_{i=1}\mathcal{L}_{per}(\hat{x}^i_{u,g}, \hat{x}^i_{s,g}).
\end{align}

In summary, our final objective is:
\begin{align}
\mathcal{L} = \mathcal{L}_{local} + \lambda_{adj}\mathcal{L}_{adj} + \lambda_{global}\mathcal{L}_{global}.
\end{align}






